Intersection cohomology of moduli spaces of vector bundles over curves

We compute the intersection cohomology of the moduli spaces $M_{r,d}$ of semistable vector bundles having rank $r$ and degree $d$ over a curve. We do this by relating the Hodge-Deligne polynomial of the intersection cohomology of $M_{r,d}$ to the Donaldson-Thomas invariants of the curve. These invariants can be computed by methods going back to Harder, Narasimhan, Desale and Ramanan. More generally, we introduce Donaldson-Thomas classes in the Grothendieck group of mixed Hodge modules over $M_{r,d}$ and relate them to the class of the intersection complex of $M_{r,d}$. Our methods can be applied to the moduli spaces of semistable objects in arbitrary hereditary categories.

==> commands_new.tex <==
\RequirePackage{amsmath,amssymb,amsthm}
\RequirePackage{etoolbox,bbm,xspace,scalerel}
\RequirePackage{version,xparse}
%\RequirePackage[a4paper,margin=1.35in]{geometry}
\makeatletter

%%%% Theorem environments
\ifx\theorem\undefined
\theoremstyle{plain}
\newtheorem{theorem}{Theorem}[section]
\newtheorem{proposition}[theorem]{Proposition}
\newtheorem{lemma}[theorem]{Lemma}
\newtheorem{corollary}[theorem]{Corollary}
\newtheorem{claim}[theorem]{Claim}
\newtheorem{conjecture}{Conjecture}
\theoremstyle{definition}
\newtheorem{remark}[theorem]{Remark}
\newtheorem{definition}[theorem]{Definition}
\newtheorem{example}[theorem]{Example}
\newtheorem{exercise}[theorem]{Exercise}
\newtheorem{question}[theorem]{Question}
\theoremstyle{remark}
\newtheorem{rmr}[theorem]{Remark}
\fi


%%%% Auxiliary commands
\def\mat#1{\ensuremath{#1}\xspace}
\def\dmat#1#2{\gdef#1{\mat{#2}}} %define math command
\def\csdmat#1#2{\csdef{#1}{\mat{#2}}}
\def\opn{\operatorname}
\def\opr#1#2{\dmat#1{\opn{#2}}}
\def\DMO{\opr}
\def\csopr#1#2{\csdmat{#1}{\opn{#2}}}
\def\oper#1{\csopr{#1}{#1}}
\def\operl{\forcsvlist\oper}
\def\redef#1{\csletcs{t@#1}{#1}\csdmat{#1}{\csuse{t@#1}}}
\newcommand\envalias[2]{\newenvironment{#1}{\begin{#2}}{\end{#2}}}


%%%% Operators. Usage: \GL
\forcsvlist\oper{
Vect,Mod,Rep,Ab,Grp,Com,Set,Top,Sch,Coh,Qcoh,Ob,Ring,Alg,
Map,Hom,End,Aut,Ext,Cat,Sh,Ind,RHom,Fun,Var,rad,
Ker,Im,Re,deg,Tr,det,rk,diag,im,coker,tr,cone,add,
sk,cosk,colim,Res,Gal,Coker,dlog,sgn,Li,
GL,SL,PGL,Gr,Lib,Conv,Sol,Tor,
Max,Spec,Proj,Ass,Ann,Quot,Pic,Sym,MHS,MHM,
td,Td,ch,Supp,supp,vol,trdeg,lc,NS,Loc,Iso,per,gr,Der,Lie,
Log,Exp,Pow,ord,lcm,VB,Hilb,cl,SU,SO,Ad,ad,id,Span,Arg,Bl,wt,Cone,
coim,Coim,eq,coeq,Eq,Coeq}

\opr\Id{id}
\opr\lHom{\lb{Hom}}
\opr\lEnd{\lb{End}}
\opr\lAut{\lb{Aut}}
\opr\lIso{\lb{Isom}}
\opr\hgt{ht}
\opr\chr{char}
\opr\udim{\mathbf{dim}}
\opr\cls{\mathsf{cl}}
\opr\mmod{mod}
\opr\Et{\mathsf{Et}}
\def\sign{\sgn}
\opr\spn{span}

\dmat\Gm{\mathbb G_{\mathrm m}}
\dmat\pt{\mathbf{pt}}
\def\opfrak#1{\csdef{#1}{\mathfrak{#1}}}
\forcsvlist\opfrak{gl,sl,su,so}
\def\oprm#1{\csdef{#1}{\mathrm{#1}}}
\forcsvlist\oprm{op,nil,et,sep,ab,top,tf,}
\def\st{\mathrm{s}}
\def\sst{\mathrm{ss}}
\def\Ta{T^{\mathrm a}} %tensor algebra
\def\Tc{T^{\mathrm c}} %tensor coalgebra
\def\Vecf{\Vect_{\mathrm f}}

%%%% Arrows
\def\mto{\mapsto}
\def\xto{\xrightarrow}
\def\lto{\leftarrow}
\def\emb{\hookrightarrow}
\def\lemb{\hookleftarrow}
\def\onto{\twoheadrightarrow}
\def\isoto{\xto{\,\smash{
	\raisebox{-3pt}{\ensuremath{\scriptstyle\sim}}
}\,}}
\RequirePackage{mathtools}
\def\xmto{\xmapsto}
\def\xlto{\xleftarrow}
\def\xemb{\xhookrightarrow}
\def\xonto#1{\xto{#1}\mathrel{\mkern-14mu}\to}
\def\dashto{\dashrightarrow}
\def\dto{\dashrightarrow}
\def\dashlto{\dashlefttarrow}
\def\dlto{\dashlefttarrow}

%%% Symbols
\dmat\es{\varnothing}%{\emptyset}
\def\bs{\backslash}
\def\ms{\backslash}
\def\sbs{\subset}
\def\sps{\supset}
\def\sbe{\subseteq}
\def\spe{\supseteq}
\redef{iff}
\dmat\imp{\implies}
\dmat\xx{\times}
\dmat\dd{\partial}
\def\pd#1{\frac\dd{\dd#1}}
\def\iso{\simeq}
\def\isoc{\cong} %canonical isomorphism
\def\bop{\bigoplus}
\def\ilim{\varprojlim} %inverse limit
\def\dlim{\varinjlim} %direct limit
\def\ts{\otimes}
\def\bts{\bigotimes}
\def\lb{\underline}
\def\ub{\overline}
\def\ubar#1{\mkern1.5mu\overline%
	{\mkern-1.5mu#1\mkern-1.5mu}\mkern1.5mu}
\def\oh{{\frac12}}
\def\toh{{\tfrac12}}
\dmat\one{\mathbbm1}
\def\qt{\delimiter"502F30E\mathopen{}} %/correct spacing
\def\partof{\vdash}
\def\adj{\mathrel{\tikz
\draw[line cap=round](0,0)--(0,1.5ex)(0,.75ex)--(-1.5ex,.75ex);}}
%\def\adj{\mathrel{\relbar\mkern-14mu\vcenter{\hbox{$\dashv$}}}}
\def\what{\widehat}
\def\tl{\tilde}
\def\wtl{\widetilde}
\def\inv{^{-1}}
\def\trp{^{\mathsf T}} %transpose
\dmat\bul{\bullet}
\def\GIT{/\!\!/}
\def\git{\GIT}
\def\qbinom{\genfrac{[}{]}{0pt}{}}
\def\ac{{\tiny\raisebox{2pt}{\textup{!`}}}}%anti-shriek
\def\m{\wedge}
\def\j{\vee}
\def\blank{\scalebox{.8}{$-$}} %blank argument

\def\upc{\tikz{\draw[->,>=latex'](0,0)--(0,.3)}}
%requires \usetikzlibrary{arrows}
\def\upc#1{\left\uparrow#1\right.}%upper closure
\def\loc#1{\left\downarrow#1\right.}%lower closure
\def\cupp{\!\smallsmile\!} %cup product
\def\capp{\!\smallfrown\!} %cap product

\NewDocumentCommand\cscale{O{.7}O{0pt}m}
%Central scale: #1-scale, #2-raise, #3-argument
{\mathbin{\ThisStyle{\vcenter{\hbox{%
  \raisebox{#2}{\scalebox{#1}{$\SavedStyle#3$}}%
}}}}}

\def\sbul{\cscale[.7][1pt]{\bullet}}
\def\dual{^{\scalerel*\vee*}}
%\def\dual{^{\cscale[.8]{\vee}}}



\usepackage[T2A]{fontenc} %T2A, OT2
\def\sha{\mathbin{\textup\cyrsh}}

\let\t@sum\sum
\def\sum{\@ifstar{\t@sum\nolimits}\t@sum}

\newcommand\tcd[2][]{%
  \begin{tikzcd}[#1,ampersand replacement=\&]#2\end{tikzcd}}

\newenvironment{ctikzcd}
	{\center\tikzcd}{\endtikzcd\endcenter}

\newcommand\edge[2][1.5em]{%\xrightarrow without tip
  \tcd[cramped,column sep=#1]{\rar[-,"#2"]\&{}}}

%%%% Aphabets: \bA,\cA,\fA,\bfA,\sA
\def\flist#1#2{\expandafter\forcsvlist\expandafter#1\expandafter{#2}}
\def\defbb#1{\csdmat{b#1}{\mathbb{#1}}}
\def\defcal#1{\csdmat{c#1}{\mathcal{#1}}}
\def\deffrak#1{\csdmat{f#1}{\mathfrak{#1}}}
\def\defbf#1{\csdmat{bf#1}{\mathbf{#1}}}
\def\defsf#1{\csdmat{s#1}{\mathsf{#1}}}
\def\defrm#1{\csdmat{r#1}{\mathrm{#1}}}
\def\defall#1{\defbb{#1}\defcal{#1}\deffrak{#1}\defbf{#1}%
  \defsf{#1}\defrm{#1}}

\forcsvlist\defall{A,B,C,D,E,F,G,H,I,J,K,L,M,N,O,P,Q,R,S,T,U,V,W,X,Y,Z}
\forcsvlist\deffrak{a,b,c,d,e,f,g,h,j,k,l,m,n,o,p,q,r,s,t,u,v,w,x,y,z}

\def\deflbf#1{\csdmat{b#1}{\mathbf{#1}}} %lower case bf
\forcsvlist\deflbf{a,b,c,d,e,g,h,i,j,k,l,n,o,p,q,r,s,t,u,v,w,x,y,z}
\forcsvlist\defbf{f,k,m} %\bff,\bfk,\bfm
%\dmat\bk{\mathbbm k}
\dmat\bk{\Bbbk}
\defrm{i} %\ri

%%%% Greek letters
\dmat\al\alpha
\dmat\be\beta
\dmat\ga\gamma
\dmat\de\delta
\dmat\la\lambda
\dmat\ta\tau
\dmat\hi\chi
\dmat\eps\varepsilon
\dmat\ep\epsilon
\dmat\io{\iota}
\dmat\vi\phi
\dmat\te\theta
\dmat\ksi\xi
\dmat\si\sigma
\dmat\om\omega
\dmat\Ga\Gamma
\dmat\La\Lambda
\dmat\De\Delta
\dmat\Om\Omega
\dmat\Si{\Sigma}
\dmat\ze\zeta
\dmat\Te{\Theta}
\dmat\Na{\nabla}
\dmat\kp{\kappa}
\forcsvlist\redef{Phi,Psi,pi,mu,nu,rho}

%%%% Structures
\RequirePackage{mleftright} %better spaces
\def\lr#1#2#3{\mleft#1#2\mright#3}
\def\set#1{\lr\{{#1}\}}
%\def\sets#1#2{\set{#1\,\lr|{\,\vphantom{#1}#2}.}}
\def\sets#1#2{\set{#1\,\middle|\,#2}}
\def\ang#1{\lr\langle{#1}\rangle}
\def\angs#1#2{\ang{#1\col#2}}
\def\rbr#1{\lr({#1})} %round bracket
\def\sbr#1{\lr[{#1}]} %square bracket
\def\brc{\set} %curly bracket, braces
\def\cbr{\set}
\def\emp{\cdot,\cdot} %empty parameters
\def\bra#1{\langle#1|}
\def\ket#1{|#1\rangle}
\def\n#1{\left\lvert#1\right\rvert}
\def\nn#1{\left\lVert#1\right\rVert}

\def\rbig#1{\big(#1\big)}
\def\rBig#1{\Big(#1\Big)}
\def\rbigg#1{\bigg(#1\bigg)}
\def\sth#1#2{\lr.{#1}|_{#2}}

\def\nspc#1{\hspace{-2.5pt}#1\hspace{-2.5pt}}%neg. space
\def\pser#1{[\![#1]\!]} %formal power series [[#1]]
\def\lser#1{(\nspc{(#1)})} %formal Laurent series ((#1))
\def\cps#1{\{#1\}} %convergent power series
\def\cls#1{(\nspc{\cps{#1}})} %convergent Laurent series
\def\angg#1{\ang{\nspc{\ang{#1}}}}
\def\nop#1{\left.\col\nspc{#1}\col\right.}%normal oper product
\def\nop#1{\left.\col\mathrel{#1}\col\right.}
%\def\nop#1{\col\mathrel{#1}\col}


\def\matr#1{\begin{matrix}#1\end{matrix}}
\def\pmat#1{\begin{pmatrix}#1\end{pmatrix}}
\def\bmat#1{\begin{bmatrix}#1\end{bmatrix}}
\def\vmat#1{\begin{vmatrix}#1\end{vmatrix}}
\def\smatr#1{\begin{smallmatrix}#1\end{smallmatrix}}
\def\smat#1{\rbr{\smatr{#1}}}
\def\pmatv#1#2{\left(\matr{#1}
	\hspace{.5ex}\middle|\hspace{.3ex}
	\matr{#2}\right)}
\def\ov#1#2{{\substack{#1\\#2}}} % #1 over #2
%\def\eq#1{\begin{equation}#1\end{equation}} %used for equalizers


%%%% Diff
\def\br{\ \vspace{-.5ex}} %break after itemize
\def\dir#1#2{\noindent\textbf{(#1)$\implies$(#2).}}
\def\clm#1{\noindent\textbf{(#1)}\xspace} %claim, \cl should be used for classes
\def\lqq{\lq\lq}
\def\rqq{\rq\rq\xspace}
\def\qq#1{\lqq#1\rqq}
\def\tpdf{\texorpdfstring} %hyperref
\def\hl{\noindent\rule{\textwidth}{1pt}}

%%%% Words and phrases
%\def\ie{i.e.\@\xspace} %id est
%\def\eg{e.g.\@\xspace} %exempli gratia
%\def\cf{cf.\@\xspace} %confer
\def\ie{i.e.,\,} %id est
\def\eg{e.g.\ } %exempli gratia
\def\cf{cf.\ } %confer
\def\lci{l.c.i.\@\xspace}
%\def\fd{f.d.\@\xspace} % used for \mathfrak{d}
\def\etale{\'etale\xspace}
\def\qis{quism\xspace} %quasi-isomorphism
\def\wrt{with respect to\xspace}
\def\hint{\noindent\textbf{Hint:}\xspace}
\def\Wlog{Without loss of generality\xspace}
\def\tfae{the following are equivalent\xspace}
\def\nbd{neighborhood\xspace}

%%%% Citations
\def\defcite#1#2{%\defcite\moz{mozgovoy_DT}
	\DeclareDocumentCommand{#1}{o}
		{\IfValueTF{##1}{\cite[##1]{#2}}{\cite{#2}}\xspace}
}
\def\eprint#1{\href{https://arxiv.org/abs/#1}{\ttfamily#1}}

%%%% Colons
\mathchardef\col=\mathcode`:
\def\colon{\nobreak \mskip 2mu\mathpunct {}\nonscript \mkern -\thinmuskip {\col}\mskip 6muplus1mu\relax}

\RequirePackage{mathtools} %for \coloneqq
\def\ordinarycolon{\col} %used in \coloneqq and \vcentcolon

{\catcode`:=\active\makeatletter
    \gdef:{\@ifnextchar={\coloneqq\@gobble}{\colon}}}
\AtBeginDocument{\mathcode`:="8000}

\mathchardef\latexequal=\mathcode`=
{\catcode`==\active\makeatletter
    \gdef={\@ifnextchar:{\eqqcolon\@gobble}{\latexequal}}}
\AtBeginDocument{\mathcode`=="8000}


%%%% Indexed definition \idef{name}{optional name}
\DeclareDocumentCommand{\idef}{mo}{%
	\ifmmode#1\else\textit{#1}\fi%
	\IfValueTF{#2}{\index{#2}}{\index{#1}}%
}


%%% Notes
\ifx\note\undefined
\RequirePackage[framemethod=TikZ]{mdframed}
\mdfsetup{backgroundcolor=brown!10, linewidth=0, skipabove=1ex, roundcorner=5pt}

\theoremstyle{definition}
\newmdtheoremenv[innertopmargin=-2pt]{note}{Note}
\newenvironment{notes}{\begin{note}}{\end{note}}

\newenvironment{comm}[1][brown!10]
    {\begin{mdframed}[backgroundcolor=#1,innertopmargin=5pt]}
    {\end{mdframed}}
\long\def\memo#1{\comm#1\endcomm}
\def\red#1{\textcolor{red}{#1}}
\fi

%custom number side in equations, manual number: \tag{name}
\makeatletter
\def\leqnomode{\tagsleft@true\let\veqno\@@leqno}
\def\reqnomode{\tagsleft@false\let\veqno\@@eqno}
\makeatother


%custom theorem, can be used to list axioms (with labels)
\ifx\customthm\undefined
\theoremstyle{plain}
\newtheorem{innercustomthm}{}
\newenvironment{customthm}[1]
  {\def\theinnercustomthm{#1}\innercustomthm}
  {\endinnercustomthm}
\fi

% subsection command
\DeclareDocumentCommand\sec{o}{
  \IfValueTF{#1}
    {\subsection{#1}}
    {\subsection{}\hspace{-1ex}}}

% short names for theorems
\def\shortThm{
\envalias{thm}{theorem}
\envalias{thr}{theorem}
\envalias{dfn}{definition}
\envalias{lmm}{lemma}
\envalias{crl}{corollary}
\envalias{prp}{proposition}
}

\makeatother

%%%% Tikz %%%%
%\long\def\command#1{\providecommand{#1}{}\renewcommand{#1}}
\newcommand\vcenterx[1]{\ensuremath{\vcenter{\hbox{#1}}}}
\newcommand\btikz[2][]{\vcenterx{\tikz[#1]{#2}}} %base line
\newcommand\ctikz[2][]{\begin{center}\tikz[#1]{#2}\end{center}}


